CrashCar101: Procedural Generation for Damage Assessment

In this paper, we are interested in addressing the problem of damage assessment for vehicles, such as cars. This task requires not only detecting the location and the extent of the damage but also identifying the damaged part. To train a computer vision system for the semantic part and damage segmentation in images, we need to manually annotate images with costly pixel annotations for both part categories and damage types. To overcome this need, we propose to use synthetic data to train these models. Synthetic data can provide samples with high variability, pixel-accurate annotations, and arbitrarily large training sets without any human intervention. We propose a procedural generation pipeline that damages 3D car models and we obtain synthetic 2D images of damaged cars paired with pixel-accurate annotations for part and damage categories. To validate our idea, we execute our pipeline and render our CrashCar101 dataset. We run experiments on three real datasets for the tasks of part and damage segmentation. For part segmentation, we show that the segmentation models trained on a combination of real data and our synthetic data outperform all models trained only on real data. For damage segmentation, we show the sim2real transfer ability of CrashCar101.

==> Experiments_backup.tex <==
%-------------------------------------------------------------------------
\section{Experimental results}
\label{sec:experiments}

\begin{figure}[t]%
    \centering
    % \subfloat[\centering Easy examples]{{\includegraphics[width = 0.49\linewidth]{figs/Figure_5.png}}}%
    %  \subfloat[\centering Hard examples]{{\includegraphics[width=0.49\linewidth]{figs/Figure_6.png} }}%
    \includegraphics[width=\linewidth]{figs/fig_partResults_1col.pdf}
    \caption{ \small \textbf{Qualitative part segmentation results.} Shows results from training on SynCD and Pascal-Part. The difficult examples often feature inconsistent labeling, occlusion or images far out of distribution.}
    \label{fig:examples_parts}%
\end{figure}

This section presents our experimental results. We evaluate the usefulness of our SynCD dataset on two tasks: semantic part segmentation (Sec.~\ref{sec:part_experiments}) and damage segmentation (Sec.~\ref{sec:damage_experiments}). For each task, we compare the segmentation models trained on our dataset to  models trained on real images and on combinations of real and synthetic data. 

\mypar{Segmentation models.}
We use two semantic segmentation models for our two tasks that use the same architecture. We train a DeepLabV3~\cite{liang2017} model for semantic segmentation of images with a ResNet50~\cite{He_2016_CVPR} backbone, which has been pretrained on ImageNet~\cite{russakovsky15ijcv} for image classification.
%
Both models are trained with the focal loss function~\cite{focalloss}. The focal loss is a modification of the standard cross-entropy loss that assigns higher weights to hard-to-classify examples, leading to improved performance on imbalanced datasets.
%
For the task of damage segmentation, we use 6 output dimensions (5 damage types plus the background category).
For the task of part segmentation, we use either 28 or 12 output dimensions depending on the real dataset that we use to evaluate the part segmentation models (see Sec.~\ref{sec:part_experiments} for more details).

 

\mypar{Implementation details.} Unless stated otherwise, we use the following settings for all models of our two tasks.
%
The input images are resized to 256$\times$256 for the task of part segmentation and 384$\times$384 for the task of damage segmentation.
%
We use a batch size of 128 for all part segmentation models and a batch size of 64 for all damage ones.
%
For a fair comparison among all trained models, we do not perform any data augmentation while training. 
%
We train all models for 20 epochs using the Adam optimizer~\cite{kingma15iclr} with an initial learning rate of 0.0002.
%
We perform an early stopping based on the performance on the hold-out validation set. Note that each different training set has its corresponding validation set coming from the same domain.
%
All experiments were run on a single Nvidia V100 GPU. \dimpp{anything else???}

\mypar{Evaluation.}
We use the traditional mean intersection-over-union (mIoU) as our main evaluation metric for both segmentation tasks.

%In this section we will value of SynCD by conducting experiments using state of the art segmentation models, and testing on real data. Experiments will be conducted for both part segmentation and damage segmentation.

\subsection{Part Segmentation}
\label{sec:part_experiments}

\mypar{Datasets.}
We use three publicly available datasets: Pascal-Part~\cite{chen14cvpr}, UDAPART \cite{liu2022learning} and CG-PART \cite{liu2019semantic}. An overview of these datasets can be seen at the top part of Tab.~\ref{tab:data}.

\begin{figure}[t]%
    \centering
    \includegraphics[width=\linewidth]{figs/fig_damageResults.pdf}
    \caption{ \small \textbf{Qualitative damage segmentation results.}\todo{fix caption}.}
    \label{fig:examples_damage}%
\end{figure}

\begin{table*}[t]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lccccc}
\bottomrule
\rowcolor{myblue2}
 \textbf{Dataset} &
 \multicolumn{2}{c}{\textbf{UDAPART}} &
 \multicolumn{1}{c}{\textbf{PASCAL-Part}} &
 \multicolumn{2}{c}{\textbf{SYNDMG100K-Part}} \\
 \rowcolor{myblue2}
 \textbf{Parts} & \textbf{11} & \textbf{27} & \textbf{11} &\textbf{11} & \textbf{27} \\
\toprule
Pascal-Part~\cite{chen14cvpr} & 39.7 & - & 40.0 & 18.4 & -  \\
CGPART~\cite{liu2019semantic} & 25.6 & 16.1 & 9.5 & 21.9 & 5.3 \\
SYNDMG100K-Part &  37.8 & \textbf{30.0}  & 19.4  & \textbf{53.1} & \textbf{46.6} \\
SYNDMG100K-Part + Pascal-Part~\cite{chen14cvpr} & \textbf{44.8} & - & \textbf{44.0} & 46.6 & - \\
SYNDMG100K & XX.X  & XX.X  & XX.X & XX.X & XX.X \\
\bottomrule
\end{tabular}
}
\caption{\small \textbf{Part segmentation mIoU results.} We report the mIoU performance for each experiment. If possible, all 27 parts from our data was evaluated, otherwise the 11 from Pascal-Part was used \todo{fix caption}.}
\label{tab:partresults}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|cccccc}
\bottomrule
\rowcolor{myblue2}
\textbf{Test Data} & \textbf{Train Data} & \textbf{mIOU}  & \textbf{Dent} & \textbf{Scratch} & \textbf{Crack} & \textbf{Glass Shatter} & \textbf{Lamp Broken}\\
\toprule
\multirow{3}{*}{\textbf{SynCD}} & 
SynCD Train & $y_1$ & $y_2$\\
& CarDD Train & - & $y_4$ \\
& CarDD Train + SynCD Train & - & $y_8$\\
\midrule
\multirow{3}{*}{\textbf{CarDD}} & 
SynCD Train & $y_1$ & $y_2$\\
& CarDD Train & $54.1$ & $26.8$ & $17.5$ & $0.0$ & $70.6$ & $29.1$ \\
& SynCD Train + CarDD Train & $63.7$ & $42.6$ & $37.6$ & $4.26$ & $81.9$ & $45.1$\\
\bottomrule
\end{tabular}
}
\caption{\small \textbf{Damage segmentation results.} \todo{fix caption}}
\label{tab:damageresults}
\end{table*}

Pascal-Part contains part annotations for 15 Pascal VOC object categories on the Pascal VOC 2010 images~\cite{everingham10ijcv}. Following previous work~\cite{???????}, we crop cars around their bounding-boxes and keep those with at least 16,384 pixels and less than 75\% background. This results in 612 images. The ``licence plate'' category was removed due to the poor annotation and the limited representation in the dataset. The pixels corresponding to this category are labeled as ``front'' or ``back'' category depending on their location. 
%We use the original training/val/test splits for this dataset.

For the UDAPART and CG-PART images, we  merge the four wheel categories into one and the two licence plates to one to align with the part definition in our synthetic data. 
% SPLITS: Since the splits for the CG-PART are not available, we use images from four car models ...... (later.....)

\mypar{Evaluation sets.}
For evaluating our the model performance we use two test sets of real images: Pascal-Part~\cite{chen14cvpr} and  UDAPART ~\cite{liu2022learning}.
 The PASCAL-Part original test set consists of 62 test images and we evaluate our models using the annotations with 11 semantic parts. UDAPART consists of 40 images and we use the whole dataset for evaluating our models using the annotations with 27 semantic parts. To enable the training and testing across these datasets, we also evaluate models on UDAPART by merging the 27 fine-grained categories to the 11 coarser categories of Pascal-Part. 
 %
 As a reference, we also report results on our hold-out SynCD-Part synthetic test set which consists of 1,575 synthetic images.

\mypar{Training sets.}
We use four different training sets to train our models:
(a) the \textbf{Pascal-Part} training set with 490 real images, 
(b) the \textbf{CGPART}~\cite{liu2019semantic} training set with 31,448 synthetic images, 
(c) our \textbf{SynCD-Part} training set with 14,175 synthetic images, and
(d) the combination of the \textbf{SynCD-Part $+$ \textbf{Pascal-Part}} training sets (14,665 images in total).
%
We train six part segmentation models in total using these sets. We train four models, one for each training set, with 11 part categories. We also train two more models with 27 part categories when the Pascal-Part set is not used (i.e., using the sets (b) and (c)).

\mypar{Results.}
We report the results of the six trained models on our evaluation sets in Tab.~\ref{tab:partresults}. 
We observe that
the models trained on our SynCD-Part (third row) perform significantly better than the models trained on the other synthetic dataset (second row) in all real valuated set (+9.9-13.9 \% mIoU).
Even though that the CGPART training set is about double in size compared to our training set (see Tab.~\ref{tab:data}), we shows that our dataset is much better and more realistic due to our rendering procedure and the number of the different car models used (99 models in SynCD-Part vs. 6 models in CGPart).
%
Interestingly, we also observe that when evaluating on the UDAPart, the model trained only on our synthetic data (third row) performs slightly worse (only -1.9\%) than the one trained on real images only of Pascal-Part (top row).
%
Finally, we show that when combining our synthetic data with the real images of Pascal-Part (bottom row), we can train a model that yield consistently a better performance in both real dataset (+4.0-5.1\%) than the model trained on on real images only (top row).
In Fig.~\ref{fig:examples_parts}, we show qualitative test examples from both real dataset.
%and we show how the model that is trained on the combination of real plus syn, performs better.

\subsection{Damage Segmentation}
\label{sec:damage_experiments}

\mypar{Datasets.} We use the recently released CarDD dataset~\cite{cardd2022} for damages on cars. To align with the damage types of our synthetic data, we remove the category flat tires. Images containing only flat tires were filtered out and the pixels annotated as flat tires are set to background. An overview of the dataset can be seen at the bottom part of Tab.~\ref{tab:data}.

\mypar{Evaluation sets.}
We evaluate our models on two test sets: the CarDD original test set from~\cite{cardd2022} which consists of 349 real images and our SynCD hold-out test set which consists of \todo{X} synthetic images.
